Approximate Message Passing with Restricted Boltzmann Machine Priors

Approximate Message Passing (AMP) has been shown to be an excellent statistical approach to signal inference and compressed sensing problem. The AMP framework provides modularity in the choice of signal prior; here we propose a hierarchical form of the Gauss-Bernouilli prior which utilizes a Restricted Boltzmann Machine (RBM) trained on the signal support to push reconstruction performance beyond that of simple iid priors for signals whose support can be well represented by a trained binary RBM. We present and analyze two methods of RBM factorization and demonstrate how these affect signal reconstruction performance within our proposed algorithm. Finally, using the MNIST handwritten digit dataset, we show experimentally that using an RBM allows AMP to approach oracle-support performance.

==> Makefile <==
FILENAME = main
PS_FILE = $(FILENAME).ps
PDF_FILE = $(FILENAME).pdf
LOG_FILE = $(FILENAME).log

PAPERSIZE = a4
# PAPERSIZE = letter

LATEX_FILES = *.dvi *.log *.toc *.tof *.aux *.blg *.lof *.lot *.bbl
CLEAN_FILES = $(LATEX_FILES) *.bak core $(PS_FILE) $(PDF_FILE)
COMPRESS_FILES = *.tex *.bib *.sty *.eps *.ps *.fig *.m *.txt *.pgm *.bst *.cls
UNCOMPRESS_FILES = *.Z *.gz

COMPRESS_DIRS = . Tables Figures
COMPRESS = gzip -q
UNCOMPRESS = gunzip

all: main


main:

	pdflatex -jobname $(FILENAME) main
	@if grep "Warning: Citation" $(LOG_FILE); then bibtex $(FILENAME); \
	pdflatex -jobname $(FILENAME) main; fi;
	@while grep Rerun main.log; do pdflaxtex -jobname $(FILENAME) main; done;
	pdflatex -jobname $(FILENAME) main

print: main
	dvips main

clean:
	@for i in $(COMPRESS_DIRS) ; \
	do \
	(if (test -d $$i) ; \
	then cd $$i ; \
	echo "Cleaning $$i" ; \
	rm -f *~ ; \
	rm -f $(CLEAN_FILES) ; \
	fi) \
	done

compress: clean
	@for i in $(COMPRESS_DIRS) ; \
	do \
	(if (test -d $$i) ; \
	then cd $$i ; \
	echo "Compressing files in $$i" ; \
	for j in $(COMPRESS_FILES) ; \
	do \
	(if (test -f $$j) ; \
	then $(COMPRESS) $$j ; \
	fi) \
	done ; \
	fi) \
	done

uncompress:
	@for i in $(COMPRESS_DIRS) ; \
	do \
	(if (test -d $$i) ; \
	then cd $$i ; \
	echo Uncompressing files in $$i ; \
	for j in $(UNCOMPRESS_FILES) ; \
	do \
	(if (test -f $$j) ; \
	then $(UNCOMPRESS) $$j ; \
	fi) \
	done ; \
	fi) \
	done


==> amp_old.tex <==
%% Sublime LaTeXTools header %%%%%%%%%%
%%... makes my life easier -- Eric
% !TEX root = main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Loopy Belief Propagation (BP) is a powerful iterative message passing
algorithm for graphical models \cite{Pearl82,MM2009}. However, it
presents two main drawbacks when applied to highly-connected,
continuous-variable problems, as in CS:
first, the need to work with continuous probability distributions; and
second, the necessity to iterate over one such probability
distribution for each pair of variables. These problems can be
addressed by projecting the distributions onto their first two moments
and by approximating the messages, which exist on the edges of the factor graph
representation of the inference problem, by the marginals existing 
on the nodes of the factor graph. 
Applying both to BP for the CS problem, one obtains the AMP iteration.

AMP has been shown to be a very powerful algorithm for CS signal
recovery, especially in the Bayesian setting where an \emph{a priori} 
model of the unknown signal is given.  
In CS, one has the following forward model to obtain set
of $M$ observations $\mathbf{y}$,
\begin{equation}
y_{\eta} = \sum_{i=1}^N F_{\eta i} x_i + w_{\eta} \quad{\rm where}\quad 
    w_{\eta} \sim \mathcal{N}\p{0,\Delta},
\label{eq:forward_model}
\end{equation}
where $F$ is an $M\times N$ matrix,
for $M\ll N$, representing linear observations of an unknown signal
$\mathbf{x}$ which are then corrupted by an additive zero-mean white
Gaussian noise (AWGN) of variance $\Delta$. The measurement rate $\alpha = M/N$
is of particular interest in determining the difficulty of this inverse problem.
In the present work, we use subscript notation to denote the individual coefficients of vectors, i.e. $y_{\eta}$ refers to the $\eta^{th}$ coefficient of ${\bf y}$ 
and the double-subscript notation to refer to individual matrix
elements in row-column order.

We can use AMP to estimate a factorization, up to 
the first two moments, of the posterior distribution
% \begin{equation}
  $P(\mathbf{x}|F,\mathbf{y}) \propto P_0(\mathbf{x})P(\mathbf{y}|F,\mathbf{x})$,
% \end{equation}
where $P(\mathbf{y}|F,\mathbf{x})$ is
% defined by
the likelihood of an observation from the AWGN channel and
$P_0(\mathbf{x})$ is a prior on the signal. If the posterior is trivially factorized, or
if it can be approximated by a factorized distribution, one can estimate the unknown
signal by averaging over the posterior,
\begin{equation}
\hat{x}_i^{\rm MMSE} = \int{\rm d}x_i~~{x_i P(x_i | F, \mathbf{y})}, \quad \forall i,
\end{equation}
which is the minimum mean squared error (MMSE) estimate of $\mathbf{x}$. This is in
contrast to utilizing a maximum \textit{a posteriori} (MAP) approach
to the solution of this inverse problem. We refer the
reader to
\cite{DMM2009,DMM2010,Ran2011,VS2013,KrzakalaPRX2012},
%%% Have to drop one citation to keep all cites on one page
% \cite{DMM2009,DMM2010,Ran2011,KrzakalaPRX2012}
and in particular to \cite{KMS2012}, for the present notation and the
derivation of AMP from BP and now give directly the iterative form of the
algorithm. Given an estimate of the factorized posterior mean
$a_i$ and variance $c_i$ for each element of $\mathbf{x}$, a single step of AMP
iteration reads
%
\begin{eqnarray}
V^{t+1}_\eta &=& \sum_i F_{\eta i}^{2} c_i^t \, ,\label{eq:V} \\
\omega^{t+1}_\eta  &=& \sum_i F_{\eta i} a^t_i -
(y_\eta-\omega^t_\eta)\frac{V^{t+1}_\eta}{\Delta+V^{t}_\eta} \, , \label{eq:omega}\\
(\Sigma^{t+1}_i)^2 &=& \left[ \sum_\eta \frac{F^2_{\eta
      i}}{\Delta+V^{t+1}_\eta} \right]^{-1} \, ,  \label{eq:S}\\
R^{t+1}_i &=& a^t_i + (\Sigma^{t+1}_i)^2 \sum_\eta F_{\eta i}
\frac{(y_\eta - \omega^{t+1}_\eta)}{\Delta+V^{t+1}_\eta} \, .\label{eq:R}
\end{eqnarray}
% 
These terms can be interpreted as follows. The variables 
$\left\{\omega_\eta\right\}$ and $\left\{V_\eta\right\}$ represent
the first and second moments, respectively,
of the marginalized messages on the $M$ factors of the factor graph. 
The variables $\left\{R_i\right\}$ and $\left\{\Sigma_i^2\right\}$ 
represent the first and second moments, respectively, of the marginalized
messages on the $N$ signal variables of the factor graph. As such,
these represent the \emph{AMP field} on the signal, which are the
observational beliefs about the continuous factorized PDF at
each signal variable. To find the final factorized posterior of the signal,
up to the two moment approximation, we must augment this 
AMP field by the signal prior. Once the new values of $R_i$ and $\Sigma_i^2$ 
are computed, the new
estimates of the posterior mean and variance, $a_i$ and $c_i$, 
given the prior $P_0(\mathbf{x})$, are calculated as
% \begin{eqnarray}
% a_i^{t+1}  &= \int {\rm d}x \frac x{  \Zi  (R_i,\Sigma_i)} P_0(x)
% e^{-\frac{(x-R_i)^2}{2\Sigma_i^2}}, \\
% c_i^{t+1} &\defined \int {\rm d}x \frac {x^2}{    \Zi  (R_i,\Sigma_i)} P_0(x)
% e^{-\frac{(x-R_i)^2}{2\Sigma_i^2}} -f_{\mathrm{a}}^2(R_i,\Sigma_i) . 
% \label{func_ac_from_prior}
% \end{eqnarray}
% \begin{eqnarray}
%   a_i^{t+1}  &\defined \int {\rm d}x_i~~\frac{x_i}{\Zi} P_0(x_i)
%   e^{-\frac{(x_i-R_i)^2}{2\Sigma_i^2}}, \label{eq:fa} \\
%   c_i^{t+1} &\defined \int {\rm d}x_i~~\frac{x_i^2}{\Zi} P_0(x_i)
%   e^{-\frac{(x_i-R_i)^2}{2\Sigma_i^2}} - \p{a_i^{t+1}}^2, 
%   \label{eq:fc}
% \end{eqnarray}
%%%%----------
%%% Changing to normal distributions
%%%%----------
\begin{eqnarray}
  a_i^{t+1}  &\defined \int {\rm d}x_i~~\frac{x_i}{\Zi} P_0(x_i)\mathcal{N}(x_i;R_i,\Sigma_i^2), \label{eq:fa} \\
  c_i^{t+1} &\defined \int {\rm d}x_i~~\frac{x_i^2}{\Zi} P_0(x_i)\mathcal{N}(x_i;R_i,\Sigma_i^2) - \p{a_i^{t+1}}^2, 
  \label{eq:fc}
\end{eqnarray}
%%%%----------
where $\Zi = \int{\rm d}x_i~~P_0(x_i)\mathcal{N}(x_i;R_i,\Sigma_i^2)$ 
is a normalization constant, commonly referred to as 
a \emph{partition function} in statistical physics.  As seen in
Eqs. (\ref{eq:fa}) and (\ref{eq:fc}), in order to use the AMP
framework, one must know some information about the class of signals
from which $\mathbf{x}$ is drawn. Commonly in CS, we are interested in
the case where the signal $\mathbf{x}$ is
\emph{sparse}, that is, very few of its coefficients are non-zero. The concept
of sparsity implies an assumption that the amount of information
required to represent $\mathbf{x}$ is actually far less than its dimensionality
would admit. Essentially, a sparse prior on $\mathbf{x}$ is extremely informative
due to its low-entropic nature.

Much of the CS literature focuses on convex approaches to this inverse
problem.  And so, a convex $\ell_1$ norm is used as a regularizer to
bias solutions to the inverse problem towards sparsity. Within the
probabilistic framework, this corresponds to a selection of a Laplace
distribution for $P_0(x_i)$.

However, AMP is not restricted to convex priors,
but can utilize non-convex priors of arbitrary complexity. For
example, one can use a two-mode Gauss-Bernoulli (GB) prior to model sparse
signals (as was considered in detail
in \cite{Ran2011,VS2013,KrzakalaPRX2012}) such as
%%%%------------------------------------------------------------
%%%  The first way to define this problem, just starting w/ the sparse GB.
%%%  Following Angélique's prescription, we can use this as an opportunity
%%%  to define the support variables, instead.
%%%%------------------------------------------------------------
% \begin{equation}
%   P_0(\mathbf{x};\rho) = \prod_i (1-\rho)\delta\p{x_i} + \frac{\rho}{\sqrt{2\pi\sigma^2}}
%       e^{-\frac{(x_i-\mu)^2}{2\sigma^2}}.
% \label{GB}
% \end{equation}
% which we note is just one example of many possible multi-modal
% priors. In this case, the GB prior has two possible modes: a zero mode
%%%------------------------------------------------------------
% \begin{eqnarray}
%   P_0(\mathbf{x})
%   = \prod_i   P_0(x_i)
%   = \prod_i   \sum_{v_i\in\bra{0,1}} P_0(v_i)P_0(x_i|v_i),
% \end{eqnarray}
\begin{equation}
  P_0(\mathbf{x})
  = \prod_i   P_0(x_i)
  = \prod_i   \sum_{v_i\in\bra{0,1}} P_0(v_i)P_0(x_i|v_i),
\end{equation}
where we have introduced Bernoulli random variables $v_i$ such that $\expval{v_i} = \rho$,
on which the values $\bra{x_i}$ are conditioned as 
% \begin{eqnarray}
% P_0(x_i|v_i=1) &= \mathcal{N(\mu,\sigma^2)}\\
% P_0(x_i|v_i=0) &= \delta(x_i).
% \end{eqnarray}
$P_0(x_i|v_i=1) = \mathcal{N}(\mu,\sigma^2)$, 
and $P_0(x_i|v_i=0) = \delta(x_i)$, where
$\delta(\cdot)$ is the zero-centered Dirac delta distribution.
This leads to the final expression for the prior,
\begin{equation}
  P_0(\mathbf{x};\rho) = \prod_i\left( (1-\rho)\delta\p{x_i} + \frac{\rho}{\sqrt{2\pi\sigma^2}} e^{-\frac{(x_i-\mu)^2}{2\sigma^2}}\right).
\label{GB}
\end{equation}
The GB prior has two possible modes: a zero mode
and a non-zero one. If we denote the set of non-zero coefficients of
$\mathbf{x}$, those for which $v_i = 1$, 
to be the \textit{support}, then the GB prior models both
the on- and off-support probability.  For $\rho \in [0,1]$, the
distribution splits the probabilistic weight between a hard
(deterministic) constraint of $x_i = 0$ and a normal distribution for
arbitrary parameters that model the on-support coefficients. For a
fixed on-support distribution, here for fixed $\mu$ and $\sigma^2$,
the value of $\rho$ controls how informative $P_0(\mathbf{x};\rho)$
is. The more informative this prior, the fewer measurements, smaller
$\alpha$, are required in order to successfully infer $\mathbf{x}$
from $\mathbf{y}$. Of course, if $\mathbf{x}$ is not truly drawn from
$P_0(\mathbf{x};\rho)$, more measurements will be required to account
for the mismatch between the true signal and the assumed signal model,
as is the case with signals which are not truly sparse but merely
compressible.

If, rather than a fixed probability of being on-support for all sites,
we instead have a local probability for each specific site to be
on-support, we can write an independent, but non-identically distributed, prior. 
For conciseness, we refer to this property as ``non-\iid'' in the 
remainder of this paper.
We easily generalize
Eq. (\ref{GB}) to
\begin{equation}
  P_0(\mathbf{x};\bra{\rho_i})
  = \prod_i \left( (1-\rho_i)\delta\p{x_i} + \frac{\rho_i}{\sqrt{2\pi\sigma^2}}
      e^{-\frac{(x_i-\mu)^2}{2\sigma^2}} \right).
\end{equation}

This change in the prior must also be reflected in the computation of the means and variances used in in Eqs. (\ref{eq:fa}) and (\ref{eq:fc}). In fact, the partition function becomes
\begin{eqnarray}
  \Zi 
    % &= \integ{x_i}P_0(x_i;\rho_i)\mathcal{N}(x_i;\ri,\si),\nn\\
    &= (1-\rho_i) \frac{1}{\sqrt{2\pi\si}}\bexp{-\frac{\ri^2}{2\si}} \nn\\
    &\quad + \rho_i \frac{1}{\sqrt{2\pi\p{\si +\sigma^2}}}\bexp{-\frac{(\ri-\mu)^2}{2(\si+\sigma^2)}}, \nn\\
    &= (1-\rho_i) \Ziz + \rho_i \Zinz,
\end{eqnarray}
where we can write the partition using two sub-partition terms
related to the off-support ($\Ziz$) and on-support ($\Zinz$) probabilities. From this
partition function, for a given setting of $\ri$ and $\si$ (which result from the AMP
evolution), we can write the posterior means and variances, $\mathbf{a}$ and $\mathbf{c}$
according to the fixed GB prior parameters $\bra{\rho_i}$, $\mu$, and $\sigma^2$.

A nice feature of this two-mode prior is that it also admits a natural estimation of
the probability
of a particular coefficient to be on- or off-support. Specifically,
at a given point in the AMP evolution, we have
%%%%---------------------------
%%%  Using the definition of v_i, now
%%%%---------------------------
% if the support of the signal is denoted as $\supp$,
% \begin{eqnarray}
%   \ampPnz
%     &= \frac{\Zinz}{\Zi}, \quad
%   \ampPz
%     = \frac{\Ziz}{\Zi},
% \end{eqnarray}
%%%%---------------------------
$\ampPnz = \frac{\rho_i\Zinz}{\Zi}$ and $\ampPz = \frac{(1-\rho_i)\Ziz}{\Zi}$, leading to
% We can write this as a Bernoulli distribution in terms of the ratio between the 
% on- and off-support probabilities for a parameter $v_i \in \bra{0,1}$ as
\begin{eqnarray}
  P^{\amp}_i(v_i) 
    &= \p{\frac{\Zinz}{\Zi}}^{v_i}\p{\frac{\Ziz}{\Zi}}^{1-v_i},\nn\\
    % &= \bexp{v_i\ln\frac{\Zinz}{\Zi} - (1-v_i)\ln\frac{\Ziz}{\Zi}},\nn\\
    &= \bexp{v_i\ln\frac{\Zinz}{\Ziz} + \ln\p{\frac{\Ziz}{\Zi}}},\nn\\
    &\propto e^{v_i\ln\gi},
    \label{eq:amp_field}
\end{eqnarray}
where
$\gi = \frac{\Zinz}{\Ziz}$ has the natural logarithm
\begin{eqnarray}
  \ln\gi 
  &= \frac{\ri^2}{2\si} - \frac{(\ri-\mu)^2}{2(\si+\sig^2)}
  + \ln\sqrt{\frac{\si}{\si+\sig^2}}. %+ \ln\frac{\rho_i}{1-\rho_i}.
\label{eq:log_gi}
\end{eqnarray}
The additional
information provided by AMP results in a
modified support probability 
$\tilde{P}(\mathbf{v})\propto P(\mathbf{v}) \prod_i e^{v_i \ln \gi}$. 
% Assuming that one can estimate a factorization of $P(\mathbf{v})$, one is
% finally able to
%
%
%%% Old
%The next question is, of course: how does one choose
% $P(v_i)$?  We propose the use of a binary RBM.  Indeed, there has been some activity in
% developing iterative algorithms with structured, non-factorized,
% priors \cite{rangan2011hybrid,schniter2010turbo,dremeau2012boltzmann}.
% We continue along this path by incorporating an RBM prior into AMP in
% Section \ref{sec:rbmamp_all}, effectively working with the factor graph defined in Fig.
% \ref{fig:factorgraph}.
%%%%--------------------------------------------------------------------------------
%%%  Angélique's original paragraph, too long
%%%%--------------------------------------------------------------------------------
% Explicating the variable $\mathbf{v}$ allows us to envisage different prior models 
% for the support of the coefficients of $\mathbf{x}$. The particular use of Bernoulli 
% laws assumes the independence between the coefficients of $\mathbf{x}$. Yet, the 
% existence of \emph{structures}, now well-acknowledged in many natural signals, 
% could be favorably taken into account through more involved models. This point of 
% view relates to the so-called \emph{structured sparsity} and has been handled in 
% numerous contributions. In the variational Bayesian context, we can cite the works 
% \cite{rangan2011hybrid,schniter2010turbo,dremeau2012boltzmann}, which respectively 
% consider a ``Group-sparsity'' through the introduction of neighborhood probabilities, 
% a Markov chain and a so-called \emph{Boltzmann machine} as a generic model. In the 
% continuation of these contributions, we propose in this paper the use of a binary 
% \emph{restricted Boltzmann machine} (RBM). In contrast with the two first latter 
% contributions, we show that this model leads to a finer modeling of the dependencies 
% between the coefficients of $\mathbf{x}$. This comes together with a low computational 
% cost of its parameter learning, which constitutes the main bottleneck of the Boltzmann 
% machine considered in \cite{dremeau2012boltzmann}. Section \ref{sec:rbm} details the 
% model and the variational approximations considered to incorporate it into the AMP 
% algorithm (Section \ref{sec:rbmamp_all}).
%%%%--------------------------------------------------------------------------------
%%%%--------------------------------------------------------------------------------
%%%  Shortening Angélique's original paragraph.
%%%%--------------------------------------------------------------------------------
Explicating 
% the variable $\mathbf{v}$ 
$P(\mathbf{v})$
allows us to envision more complex support models 
for the coefficients of $\mathbf{x}$. The previous model
assumes the independence between the coefficients of $\mathbf{x}$, however, the 
existence of dependencies, now well-acknowledged for many natural signals
as \emph{structured sparsity}, can be leveraged through joint models. 
In the variational Bayesian context, we cite
\cite{rangan2011hybrid,schniter2010turbo,dremeau2012boltzmann}, which
consider neighborhood probabilities, Markov chains, and so-called 
\emph{Boltzmann machines}, respectively, as generic support models.
In similar vein, we propose the use of a binary 
RBM as a joint support model. In contrast with the models of 
\cite{rangan2011hybrid,schniter2010turbo}, the RBM model can provide
a more accurate modeling of support correlations. Also, the RBM model can
be trained at low cost \cite{Hin2002}, which is the main bottleneck of the \emph{general}
Boltzmann machine model used in \cite{dremeau2012boltzmann}.
% In contrast with \cite{rangan2011hybrid,schniter2010turbo}, 
% we show that this model better accounts for the dependencies 
% between the coefficients of $\mathbf{x}$. 
% This comes together with a low computational 
% cost of its parameter learning, which constitutes the main bottleneck of the Boltzmann 
% machine considered in \cite{dremeau2012boltzmann}. Section \ref{sec:rbm} details the 
% model and the variational approximations considered to incorporate it into the AMP 
% algorithm (Section \ref{sec:rbmamp_all}).
%%%%--------------------------------------------------------------------------------

==> fig_mcc_quad.tex <==
\begin{figure}
\centering
	\includegraphics[width=0.24\textwidth]{figures/csrecon_a015_mcc.png}~
	\includegraphics[width=0.24\textwidth]{figures/csrecon_a025_mcc.png}\\
	\includegraphics[width=0.24\textwidth]{figures/csrecon_a035_mcc.png}~
	\includegraphics[width=0.24\textwidth]{figures/csrecon_a045_mcc.png}\\
\caption{\label{fig:quad_mcc}
		Comparison over tested MNIST handwritten digits for support detection
		performance in terms of MCC for 
		$\alpha = 0.15$ (top left), 
		$\alpha = 0.25$ (top right),
		$\alpha = 0.35$ (bottom left), and
		$\alpha = 0.45$ (bottom right). 
		Black curve: AMP using GB prior.
		Red curve: AMP using RBM (MF) support prior.
		Blue curve: AMP using RBM (TAP) support prior.
		}
\end{figure}

==> fig_nsnr_quad.tex <==
\begin{figure}
\centering
	\includegraphics[width=0.24\textwidth]{figures/csrecon_a015_nsnr.png}~
	\includegraphics[width=0.24\textwidth]{figures/csrecon_a025_nsnr.png}\\
	\includegraphics[width=0.24\textwidth]{figures/csrecon_a035_nsnr.png}~
	\includegraphics[width=0.24\textwidth]{figures/csrecon_a045_nsnr.png}\\
\caption{\label{fig:allrecons}
		Comparison over tested MNIST handwritten digits for reconstruction
		performance in terms of NSNR for 
		$\alpha = 0.15$ (top left), 
		$\alpha = 0.25$ (top right),
		$\alpha = 0.35$ (bottom left), and
		$\alpha = 0.45$ (bottom right). 
		Black curve: AMP using GB prior.
		Red curve: AMP using RBM (MF) support prior.
		Blue curve: AMP using RBM (TAP) support prior.
		}
\end{figure}

==> fig_viscompare.tex <==
\fboxsep=0mm%padding thickness
\fboxrule=2pt%border thickness

\begin{figure}
\centering
	\includegraphics[width=0.15\textwidth]{figures/demoimg_orig.png}\\
	Original Image ($\rho = 0.388$)\\
	% \belowspace

	% At \alpha = 0.15
	\fcolorbox{red}{red}{\includegraphics[width=0.15\textwidth]{figures/demoimg_gb_a015.png}}~
	\fcolorbox{red}{red}{\includegraphics[width=0.15\textwidth]{figures/demoimg_rbmmf_a015.png}}~
	\fcolorbox{red}{red}{\includegraphics[width=0.15\textwidth]{figures/demoimg_rbmtap_a015.png}}\\
	\vskip 0.12in
	
	% At \alpha = 0.25
	\fcolorbox{red}{red}{\includegraphics[width=0.15\textwidth]{figures/demoimg_gb_a025.png}}~
	\fcolorbox{red}{red}{\includegraphics[width=0.15\textwidth]{figures/demoimg_rbmmf_a025.png}}~
	\fcolorbox{red}{red}{\includegraphics[width=0.15\textwidth]{figures/demoimg_rbmtap_a025.png}}\\
	\vskip 0.12in
	
	% At \alpha = 0.35
	\fcolorbox{red}{red}{\includegraphics[width=0.15\textwidth]{figures/demoimg_gb_a035.png}}~
	\fcolorbox{green}{green}{\includegraphics[width=0.15\textwidth]{figures/demoimg_rbmmf_a035.png}}~
	\fcolorbox{green}{green}{\includegraphics[width=0.15\textwidth]{figures/demoimg_rbmtap_a035.png}}\\	
	\vskip 0.12in
	
	% At \alpha = 0.45
	\fcolorbox{red}{red}{\includegraphics[width=0.15\textwidth]{figures/demoimg_gb_a045.png}}~
	\fcolorbox{green}{green}{\includegraphics[width=0.15\textwidth]{figures/demoimg_rbmmf_a045.png}}~
	\fcolorbox{green}{green}{\includegraphics[width=0.15\textwidth]{figures/demoimg_rbmtap_a045.png}}\\	
	\vskip 0.12in
	
	% At \alpha = 0.55
	\fcolorbox{green}{green}{\includegraphics[width=0.15\textwidth]{figures/demoimg_gb_a055.png}}~
	\fcolorbox{green}{green}{\includegraphics[width=0.15\textwidth]{figures/demoimg_rbmmf_a055.png}}~
	\fcolorbox{green}{green}{\includegraphics[width=0.15\textwidth]{figures/demoimg_rbmtap_a055.png}}\\	
	% \belowspace

	\caption{\label{fig:visualcompare}
		Reconstruction of a sample image of digit ``3''
		for different subrates 
		(Top to Bottom: $\alpha = 0.15$, $0.25$, $0.35$, $0.45$, and $0.55$).
		Left Column: reconstruction using AMP with GB prior. 
		Middle Column: reconstruction using AMP with RBM (MF).
		Right Column: reconstruction using AMP with RBM (TAP).
		Failed reconstructions ($> -15$~dB NSNR) are indicated with red borders,
		while successful reconstructions ($\leq-15$~dB NSNR) are indicated
		with green borders.
	}

\end{figure}

==> table_sparsity.tex <==
\begin{table}[t]
	% \caption{Average sparsity for classes of handwritten digits in
	%          the tested subset of the MNIST database sorted}
	\caption{Classes of handwritten digits in the tested subset of 
	the MNIST database sorted according to the average sparsity of 
	each digit class. The average sparsity is reported along with
	the standard deviation of the sparsity across all samples of
	the digit class. }
    \label{tab:sparsity}
	\vskip 0.15in
	\begin{center}
	\begin{small}
	\begin{sc}
	\begin{tabular}{c|c}
	\hline
	% \abovespace\belowspace
	Digit Class &  $\rho$ \\
	\hline
	% \abovespace
		 ``1'' &  $0.200 \pm 0.050$ \\
		 ``7'' &  $0.277 \pm 0.064$ \\
		 ``9'' &  $0.309 \pm 0.069$ \\
		 ``4'' &  $0.313 \pm 0.067$ \\
		 ``5'' &  $0.321 \pm 0.078$ \\
		 ``6'' &  $0.340 \pm 0.076$ \\
		 ``3'' &  $0.362 \pm 0.085$ \\
		 ``2'' &  $0.373 \pm 0.082$ \\		 		 		 		 		 		 
		 ``8'' &  $0.377 \pm 0.076$ \\
		 ``0'' &  $0.441 \pm 0.086$ \\
	 \hline
	% \belowspace
	% Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& $\surd$ \\
	% \hline
	\end{tabular}
	\end{sc}
	\end{small}
	\end{center}
	\vskip -0.1in
\end{table}

==> table_sr_all.tex <==
\begin{table}[t]
	\caption{Reconstruction success rates for the handwritten digit test set
			 over measurement rate for different classes of digits. 
			 A successful reconstruction is denoted as
			 a reconstruction which acheives an NSNR $\leq -15$~dB.}
    \label{tab:sr_all}
	\vskip 0.15in
	\begin{center}
	\begin{small}
	\begin{sc}
	\begin{tabular}{l|lcccc}
	% \multicolumn{1}{c}{~} & \multicolumn{4}{c}{$\alpha$} \\
	\hline	
		All Digits &  $\alpha$ & 0.15 &  0.25 &  0.35 & 0.45 \\
	\hline
		GB        &~& 0.0\% & 0.5\% & 11.3\% & 50.6\% \\ 
		RBM (MF)  &~& 0.1\% & 10.6\% & 53.6\% & 88.7\% \\ 
		RBM (TAP) &~& 0.1\% & 14.7\% & 58.9\% & 88.1\% \\ 
	\hline
	 	``1'' Digits  &  $\alpha$ &  0.15 &  0.25 &  0.35 & 0.45 \\
	\hline
		GB        &~& 0.0\% & 3.5\% & 61.1\% & 99.1\% \\ 
		RBM (MF)  &~& 0.9\% & 51.3\% & 92.9\% & 100.0\% \\ 
		RBM (TAP) &~& 0.9\% & 69.9\% & 98.2\% & 100.0\% \\ 
	\hline
	 	``7'' Digits &  $\alpha$ &  0.15 &  0.25 &  0.35 & 0.45 \\
	\hline
		GB        &~& 0.0\% & 0.0\% & 16.4\% & 79.5\% \\ 
		RBM (MF)  &~& 0.0\% & 23.0\% & 88.5\% & 100.0\% \\ 
		RBM (TAP) &~& 0.0\% & 27.9\% & 93.4\% & 100.0\% \\ 
	\hline
	 	``5'' Digits &  $\alpha$ &  0.15 &  0.25 &  0.35 & 0.45 \\
	\hline
		GB &~ & 0.0\% & 0.0\% & 9.2\% & 62.1\% \\ 
		RBM (MF) &~ & 0.0\% & 1.1\% & 52.9\% & 94.3\% \\ 
		RBM (TAP) &~ & 0.0\% & 5.7\% & 65.5\% & 94.3\% \\ 	
	\hline
	 	``2'' Digits &  $\alpha$ &  0.15 &  0.25 &  0.35 & 0.45 \\
	\hline
		GB        &~& 0.0\% & 0.0\% & 2.1\% & 33.0\% \\ 
		RBM (MF)  &~& 0.0\% & 3.2\% & 21.3\% & 83.0\% \\ 
		RBM (TAP) &~& 0.0\% & 3.2\% & 34.0\% & 83.0\% \\ 
	\hline
	 	``0'' Digits &  $\alpha$ &  0.15 &  0.25 &  0.35 & 0.45 \\
	\hline
		GB        &~& 0.0\% & 0.0\% & 0.0\% & 7.4\% \\ 
		RBM (MF)  &~& 0.0\% & 0.0\% & 14.9\% & 55.3\% \\ 
		RBM (TAP) &~& 0.0\% & 0.0\% & 16.0\% & 53.2\% \\ 
	\hline
	\end{tabular}
	\end{sc}
	\end{small}
	\end{center}
	\vskip -0.1in
\end{table}

==> table_srsupp_all.tex <==
\begin{table}[t]
	\caption{Support recovery success rates for the handwritten digit test set
			 over measurement rate for different classes of digits. 
			 A successful support reconstruction is denoted as
			 a reconstruction which acheives an $\text{MCC} \geq 0.70$ when
			 compared to the true support.}
    \label{tab:srsupp_all}
	\vskip 0.15in
	\begin{center}
	\begin{small}
	\begin{sc}
	\begin{tabular}{l|lcccc}
	% \multicolumn{1}{c}{~} & \multicolumn{4}{c}{$\alpha$} \\
	\hline	
		All Digits &  $\alpha$ & 0.15 &  0.25 &  0.35 & 0.45 \\
	\hline
GB  &~& 0.0\% & 0.5\% & 12.1\% & 52.0\% \\ 
RBM (MF) &~& 12.4\% & 60.8\% & 92.4\% & 99.9\% \\ 
RBM (TAP)  &~& 24.6\% & 76.9\% & 98.1\% & 100.0\% \\ 

	\hline
	 	``1'' Digits  &  $\alpha$ &  0.15 &  0.25 &  0.35 & 0.45 \\
	\hline
GB  &~& 0.0\% & 3.5\% & 61.1\% & 99.1\% \\ 
RBM (MF) &~& 12.4\% & 69.0\% & 92.9\% & 100.0\% \\ 
RBM (TAP)  &~& 29.2\% & 86.7\% & 98.2\% & 100.0\% \\ 

	\hline
	 	``7'' Digits &  $\alpha$ &  0.15 &  0.25 &  0.35 & 0.45 \\
	\hline
GB  &~& 0.0\% & 0.0\% & 18.9\% & 79.5\% \\ 
RBM (MF) &~& 13.9\% & 77.0\% & 96.7\% & 100.0\% \\ 
% \belowspace
RBM (TAP)  &~& 38.5\% & 89.3\% & 100.0\% & 100.0\% \\ 

	\hline
	 	``5'' Digits &  $\alpha$ &  0.15 &  0.25 &  0.35 & 0.45 \\
	\hline
GB  &~& 0.0\% & 0.0\% & 10.3\% & 63.2\% \\ 
RBM (MF) &~& 3.4\% & 29.9\% & 79.3\% & 100.0\% \\ 
RBM (TAP)  &~& 3.4\% & 60.9\% & 94.3\% & 100.0\% \\  

	\hline
	 	``2'' Digits &  $\alpha$ &  0.15 &  0.25 &  0.35 & 0.45 \\
	\hline
GB  &~& 0.0\% & 0.0\% & 2.1\% & 33.0\% \\ 
RBM (MF) &~& 5.3\% & 43.6\% & 83.0\% & 100.0\% \\ 
RBM (TAP)  &~& 10.6\% & 63.8\% & 97.9\% & 100.0\% \\ 

	\hline
	 	``0'' Digits &  $\alpha$ &  0.15 &  0.25 &  0.35 & 0.45 \\
	\hline
GB  &~& 0.0\% & 0.0\% & 0.0\% & 9.6\% \\ 
RBM (MF) &~& 22.3\% & 70.2\% & 94.7\% & 100.0\% \\ 
RBM (TAP)  &~& 36.2\% & 80.9\% & 97.9\% & 100.0\% \\ 

	\hline
	\end{tabular}
	\end{sc}
	\end{small}
	\end{center}
	\vskip -0.1in
\end{table}
